Bayesian Nonparametric Estimation for Point Processes with Spatial Homogeneity: A Spatial Analysis of NBA Shot Locations

Basketball shot location data provide valuable summary information regarding players to coaches, sports analysts, fans, statisticians, as well as players themselves. Represented by spatial points, such data are naturally analyzed with spatial point process models. We present a novel nonparametric Bayesian method for learning the underlying intensity surface built upon a combination of Dirichlet process and Markov random field. Our method has the advantage of effectively encouraging local spatial homogeneity when estimating a globally heterogeneous intensity surface. Posterior inferences are performed with an efficient Markov chain Monte Carlo (MCMC) algorithm. Simulation studies show that the inferences are accurate and that the method is superior compared to the competing methods. Application to the shot location data of $20$ representative NBA players in the 2017-2018 regular season offers interesting insights about the shooting patterns of these players. A comparison against the competing method shows that the proposed method can effectively incorporate spatial contiguity into the estimation of intensity surfaces.

==> Makefile <==
source := spp_grf.tex # $(wildcard *.tex)
out := $(patsubst %.tex,%.pdf,$(source))
rev := 56a50ce
latest := $(shell git log --format="%h" | head -n 1)
bib := $(wildcard *.bib)

.PHONY: all
all: $(out)

%.pdf: %.tex $(bib)
	@latexmk -pdf $<
#	@latexmk -c

## compare modification with the latest version checked into git
## for comparison of specific commits:
##	latexdiff-vc --git -r old_githash -r new_githash --pdf source.tex
diff:
	latexdiff-vc --git --pdf --force $(source) -r $(rev)

log:
	@git log --pretty=format:"%h by %an at %ar: %s" $(source) | head -n 15

.PNONY: clean
clean:
	rm -rf $(out)\
	  *~ .*~ .\#* .Rhistory *.aux *.bbl *.blg *.out *.log *.toc\
	  *.fff *.fdb_latexmk *.fls *.ttt *diff* *oldtmp*

